Sobolev spaces associated to singular and fractional Radon transforms

The purpose of this paper is to study the smoothing properties (in $L^p$ Sobolev spaces) of operators of the form $f\mapsto \psi(x) \int f(\gamma_t(x)) K(t)\: dt$, where $\gamma_t(x)$ is a $C^\infty$ function defined on a neighborhood of the origin in $(t,x)\in\mathbb{R}^N\times \mathbb{R}^n$, satisfying $\gamma_0(x)\equiv x$, $\psi$ is a $C^\infty$ cut-off function supported on a small neighborhood of $0\in \mathbb{R}^n$, and $K$ is a "multi-parameter fractional kernel" supported on a small neighborhood of $0\in \mathbb{R}^N$. When $K$ is a Calder\'on-Zygmund kernel these operators were studied by Christ, Nagel, Stein, and Wainger, and when $K$ is a multi-parameter singular kernel they were studied by the author and Stein. In both of these situations, conditions on $\gamma$ were given under which the above operator is bounded on $L^p$ ($1<p<\infty$). Under these same conditions, we introduce non-isotropic $L^p$ Sobolev spaces associated to $\gamma$. Furthermore, when $K$ is a fractional kernel which is smoothing of an order which is close to $0$ (i.e., very close to a singular kernel) we prove mapping properties of the above operators on these non-isotropic Sobolev spaces. As a corollary, under the conditions introduced on $\gamma$ by Christ, Nagel, Stein, and Wainger, we prove optimal smoothing properties in isotropic $L^p$ Sobolev spaces for the above operator when $K$ is a fractional kernel which is smoothing of very low order.

==> revistabbl.tex <==
%\providecommand{\bysame}{\leavevmode\hbox to3em{\hrulefill}\thinspace}
%\providecommand{\MR}{\relax\ifhmode\unskip\space\fi MR }
% \MRhref is called by the amsart/book/proc definition of \MR.
%\providecommand{\MRhref}[2]{%
%  \href{http://www.ams.org/mathscinet-getitem?mr=#1}{#2}
%}
%\providecommand{\href}[2]{#2}
%\begin{thebibliography}{10}

\bibitem{ChangNagelSteinEstaimtesForDbarNeumannProblem}
\RMIauthor{Chang, D.-C. and Nagel, A. and Stein, E.} 
\RMIpaper{Estimates for the
  {$\overline\partial$}-{N}eumann problem in pseudoconvex domains of finite
  type in {${\bf C}^2$}} 
\RMIjournal{Acta Math.} \textbf{169} (1992), no.~3-4, 153--228.
 % \MR{1194003 (93k:32025)}

\bibitem{ChangFeffermanSomeRecentDevelopmentsInFourierAnalysisAndHpTheory}
\RMIauthor{Chang, S.-Y. and Fefferman, R.} 
\RMIpaper{Some recent developments in
  {F}ourier analysis and {$H^p$}-theory on product domains}
 \RMIjournal{Bull. Amer. Math.
  Soc.} (N.S.) \textbf{12} (1985), no.~1, 1--43. 
%\MR{766959 (86g:42038)}

\bibitem{ChristHilbertTransformsAlongCurvesI}
\RMIauthor{Christ, M.} 
\RMIpaper{Hilbert transforms along curves. {I}. {N}ilpotent
  groups} 
\RMIjournal{Ann. of Math.} (2) \textbf{122} (1985), no.~3, 575--596. 
%\MR{819558}

\bibitem{ChristEndpointBoundsForSingularFractionalIntegralOperators}
\RMIauthor{Christ, M.} 
\RMIpaper{Endpoint bounds for singular fractional integral operators},
  unpublished, 1988.

\bibitem{ChirstGellerGlowackiPolinPseudodifferentialOperatorsOnGroupsWithDilations}
\RMIauthor{Christ, M. and Geller, D. and G{\l}owacki, P. and L Polin, L.}
  \RMIpaper{Pseudodifferential operators on groups with dilations} 
\RMIjournal{Duke Math. J.}
  \textbf{68} (1992), no.~1, 31--65. 
%\MR{1185817}

\bibitem{ChristNagelSteinWaingerSingularAndMaximalRadonTransforms}
\RMIauthor{Christ, M. and Nagel, A. and Stein, E. and Wainger, S.}
  \RMIpaper{Singular and maximal {R}adon transforms: analysis and geometry} 
\RMIjournal{Ann.
  of Math.} (2) \textbf{150} (1999), no.~2, 489--577. 
%\MR{MR1726701 (2000j:42023)}

\bibitem{CuccagnaSobolevEstimatesForFractionalAndSingularRadonTransforms}
\RMIauthor{Cuccagna, S.} 
\RMIpaper{Sobolev estimates for fractional and singular {R}adon
  transforms} 
\RMIjournal{J. Funct. Anal.} \textbf{139} (1996), no.~1, 94--118. 
%\MR{1399687 (98f:42010)}

\bibitem{FabesSingularIntegralsAndPartialDifferentialEquationsOfParabolicType}
\RMIauthor{Fabes, E.} 
\RMIpaper{Singular integrals and partial differential equations of
  parabolic type} 
\RMIjournal{Studia Math.} \textbf{28} (1966/1967), 81--131.
% \MR{0213744
%  (35 \#4601)}

\bibitem{FeffermanPhongSubellipticEigenValueProblems}
\RMIauthor{Fefferman, C. and Phong, D.} 
\RMIpaper{Subelliptic eigenvalue problems}
  In \RMIbook{Conference on harmonic analysis in honor of {A}ntoni {Z}ygmund, {V}ol. {I},
  {II}} ({C}hicago, {I}ll., 1981), Wadsworth Math. Ser., Wadsworth, Belmont, CA,
  1983, pp.~590--606. 
%\MR{730094 (86c:35112)}

\bibitem{FeffermanSingularIntegralsOnProductDomains}
\RMIauthor{Fefferman, R.} 
\RMIpaper{Singular integrals on product domains} 
\RMIjournal{Bull. Amer.
  Math. Soc.} (N.S.) \textbf{4} (1981), no.~2, 195--201. 
%\MR{MR598687
%  (83i:42014)}

\bibitem{FeffermanHarmonicAnalysisOnProductSpaces}
\RMIauthor{Fefferman, R.} 
\RMIpaper{Harmonic analysis on product spaces} 
\RMIjournal{Ann. of Math.} (2)
  \textbf{126} (1987), no.~1, 109--130. 
%\MR{898053 (90e:42030)}

\bibitem{FeffermanSomeRecentDevelopmentsInFourierAnalysisII}
\RMIauthor{Fefferman, R.} 
\RMIpaper{Some recent developments in {F}ourier analysis and {$H^p$}
  theory on product domains. {II}}
In \RMIbook{Function spaces and applications} ({L}und,
  1986), Lecture Notes in Math., vol. 1302, Springer, Berlin, 1988, pp.~44--51.

\bibitem{FeffermanSteinSingularIntegralsOnProductSpaces}
\RMIauthor{Fefferman, R. and Stein, E.} \RMIpaper{Singular integrals on product
  spaces} 
\RMIjournal{Adv. in Math.} \textbf{45} (1982), no.~2, 117--143.
% \MR{664621
 % (84d:42023)}

\bibitem{FollandSubellipticEstimatesAndFunctionSpacesOnNilpotent}
\RMIauthor{Folland, G.} 
\RMIpaper{Subelliptic estimates and function spaces on nilpotent
  {L}ie groups} 
\RMIjournal{Ark. Mat.} \textbf{13} (1975), no.~2, 161--207. 
%\MR{0494315 (58
 % \#13215)}

\bibitem{FollandSteinEstimatesForTheDbarComplex}
\RMIauthor{Folland, G. and Stein, E.} 
\RMIpaper{Estimates for the {$\bar \partial _{b}$}
  complex and analysis on the {H}eisenberg group} 
\RMIjournal{Comm. Pure Appl. Math.}
  \textbf{27} (1974), 429--522. 
%\MR{0367477 (51 \#3719)}

\bibitem{GellerSteinSingularConvolutionOperatorsOnTheHeisenbergGroup}
\RMIauthor{Geller, D. and Stein, E.} 
\RMIpaper{Singular convolution operators on the
  {H}eisenberg group} 
\RMIjournal{Bull. Amer. Math. Soc.} (N.S.) \textbf{6} (1982), no.~1,
  99--103. %\MR{634441}

\bibitem{GellerSteinEstimatesForSingularConvolutionOperatorsOnTheHeisenbergGroup}
\RMIauthor{Geller, D. and Stein, E.} 
\RMIpaper{Estimates for singular convolution operators on the {H}eisenberg
  group} 
\RMIjournal{Math. Ann.} \textbf{267} (1984), no.~1, 1--15. 
%\MR{737332}

\bibitem{GlowackiCompositionAndLtBoundednessOfFlagKernels}
\RMIauthor{G{\l}owacki, P.} 
\RMIpaper{Composition and {$L^2$}-boundedness of flag
  kernels} 
\RMIjournal{Colloq. Math.} \textbf{118} (2010), no.~2, 581--585. 
%\MR{2602167
 % (2011h:42015)}

\bibitem{GlowackiCompositionAndLtBoundednessOfFlagKernelsCorrection}
\RMIauthor{G{\l}owacki, P.} 
\RMIpaper{Correction to ``{C}omposition and {$L^2$}-boundedness of flag
  kernels''} 
\RMIjournal{Colloq. Math.} \textbf{120} (2010), no.~2, 331.
 % \MR{2679042 (2011h:42016)}

\bibitem{GlowackiLpBoundednessOfFlagKernelsOnHomogeneousGroups}
\RMIauthor{G{\l}owacki, P.} 
\RMIpaper{{$L^p$}-boundedness of flag kernels on homogeneous groups via
  symbolic calculus} 
\RMIjournal{J. Lie Theory} \textbf{23} (2013), no.~4, 953--977.
%  \MR{3185206}

\bibitem{GoodmanNilpotentLieGroups}
\RMIauthor{Goodman, R.} 
\RMIbook{Nilpotent {L}ie groups: structure and applications to
  analysis} Lecture Notes in Mathematics, Vol. 562, Springer-Verlag,
  Berlin-New York, 1976. i
%\MR{0442149 (56 \#537)}

\bibitem{GreenblattAnAnalogueToATheoremOfFeffermanAndPhong}
\RMIauthor{Greenblatt, M.} 
\RMIpaper{An analogue to a theorem of {F}efferman and {P}hong
  for averaging operators along curves with singular fractional integral
  kernel} 
\RMIjournal{Geom. Funct. Anal.} \textbf{17} (2007), no.~4, 1106--1138.
 % \MR{2373012 (2008m:42018)}

\bibitem{GreenleafSeegerWaingerOnXrayTransformsForRigidLineComplexes}
\RMIauthor{Greenleaf, A. and Seeger, A. and Wainger, A.} 
\RMIpaper{On {X}-ray
  transforms for rigid line complexes and integrals over curves in {${\bf R}\sp
  4$}} 
\RMIjournal{Proc. Amer. Math. Soc.} \textbf{127} (1999), no.~12, 3533--3545.
 % \MR{MR1670367 (2001a:44002)}

\bibitem{GreenleafUhlmannEstimatesForSingularRadonTransforms}
\RMIauthor{Greenleaf, A. and Uhlmann, G.} 
\RMIpaper{Estimates for singular {R}adon
  transforms and pseudodifferential operators with singular symbols}
\RMIjournal{J. Funct.
  Anal.} \textbf{89} (1990), no.~1, 202--232.
% \MR{1040963}

\bibitem{JourneCalderonZygmundOperatorsOnProductSpaces}
\RMIauthor{Journ{\'e}, J.} 
\RMIpaper{Calder\'on-{Z}ygmund operators on product spaces},
  \RMIjournal{Rev. Mat. Iberoamericana}
 \textbf{1} (1985), no.~3, 55--91. 
%\MR{836284
%  (88d:42028)}

\bibitem{KoenigOnMaximalSobolevAndHolderEstimatesForTheTangentialCR}
\RMIauthor{Koenig, K.} 
\RMIpaper{On maximal {S}obolev and {H}\"older estimates for the
  tangential {C}auchy-{R}iemann operator and boundary {L}aplacian}
\RMIjournal{Amer. J.
  Math.} \textbf{124} (2002), no.~1, 129--197. 
%\MR{MR1879002 (2002m:32061)}

\bibitem{MullerCalderonZygmundKernelsCarriedByLinearSubsubspace}
\RMIauthor{M{\"u}ller, D.}
\RMIpaper{Calder\'on-{Z}ygmund kernels carried by linear subspaces
  of homogeneous nilpotent {L}ie algebras}
\RMIjournal{Invent. Math.} \textbf{73} (1983),
  no.~3, 467--489.
% \MR{718942}

\bibitem{MullerTwistedConvolutionsWithCalderonZygmundKernels}
\RMIauthor{M{\"u}ller, D.}
\RMIpaper{Twisted convolutions with {C}alder\'on-{Z}ygmund
  kernels} 
\RMIjournal{J. Reine Angew. Math.} \textbf{352} (1984), 133--150. 
%\MR{758698}

\bibitem{MullerSingularKernelsSupportedByHomogeneousSubmanifolds}
\RMIauthor{M{\"u}ller, D.}
\RMIpaper{Singular kernels supported by homogeneous submanifolds}
\RMIjournal{J.
  Reine Angew. Math.} \textbf{356} (1985), 90--118. 
%\MR{779377}

\bibitem{MullerRicciSteinMarcinkiewiczMulipliersAndMulitparameterStructure}
\RMIauthor{M{\"u}ller, D. and Ricci, F. and Stein, E.} 
\RMIpaper{Marcinkiewicz
  multipliers and multi-parameter structure on {H}eisenberg (-type) groups.
  {I}}
\RMIjournal{ Invent. Math.} \textbf{119} (1995), no.~2, 199--233.
% \MR{1312498
%  (96b:43005)}

\bibitem{MullerRicciSteinMarcinkiewiczMultipliersAndMultiParameterStructuresOnHeisenbergTypeGroupsII}
\RMIauthor{M{\"u}ller, D. and Ricci, F. and Stein, E.} 
\RMIpaper{Marcinkiewicz multipliers and multi-parameter structure on
  {H}eisenberg (-type) groups. {II}} 
\RMIjournal{Math. Z.} \textbf{221} (1996), no.~2,
  267--291. 
%\MR{1376298 (97c:43007)}

\bibitem{NagelRosaySteinWaingerEstimatesForTheBergmanAndSzegoKernels}
\RMIauthor{Nagel, A. and Rosay, J. and  Stein, E. and Wainger, S.} 
\RMIpaper{Estimates for the
  {B}ergman and {S}zeg{\H o} kernels in {${\bf C}\sp 2$}} 
\RMIjournal{Ann. of Math.} (2)
  \textbf{129} (1989), no.~1, 113--149. %\MR{MR979602 (90g:32028)}

\bibitem{NagelRicciSteinWaingerSingularIntegralWithFlagKernelsOnHomogeneousGroupsI}
\RMIauthor{Nagel, A. and Ricci, F. and Stein, E. and Wainger, S.} \RMIpaper{Singular
  integrals with flag kernels on homogeneous groups, {I}}
\RMIjournal{Rev. Mat. Iberoam.}
  \textbf{28} (2012), no.~3, 631--722. %\MR{2949616}

\bibitem{NagelRicciSteinSingularIntegralsWithFlagKernels}
\RMIauthor{Nagel, A. and Ricci, F. and Stein, E.} \RMIpaper{Singular integrals
  with flag kernels and analysis on quadratic {CR} manifolds} 
\RMIjournal{J. Funct. Anal.}
  \textbf{181} (2001), no.~1, 29--118. %\MR{MR1818111 (2001m:22018)}

\bibitem{NagelRiviereWaingerI}
\RMIauthor{Nagel, A. and Rivi{\`e}re, N. and Wainger, S.} 
\RMIpaper{On
  {H}ilbert transforms along curves} 
\RMIjournal{Bull. Amer. Math. Soc.} \textbf{80}
  (1974), 106--108. %\MR{0450899}

\bibitem{NagelRiviereWaingerIII}
\RMIauthor{Nagel, A. and Rivi{\`e}re, N. and Wainger, S.} 
\RMIpaper{A maximal function
  associated to the curve {$(t, t^{2})$}} 
\RMIjournal{Proc. Nat. Acad. Sci. U.S.A.}
  \textbf{73} (1976), no.~5, 1416--1417. %\MR{0399389}

\bibitem{NagelRiviereWaingerII}
\RMIauthor{Nagel, A. and Rivi{\`e}re, N. and Wainger, S.} 
\RMIpaper{On
  {H}ilbert transforms along curves. {II}} 
\RMIjournal{Amer. J. Math.} \textbf{98} (1976),
  no.~2, 395--403. %\MR{0450900}

\bibitem{NagelSteinWaingerHilbertTransformsAndMaximalFunctionsRelatedToVariableCurves}
\RMIauthor{Nagel, A. and Stein, E. and Wainger, S.} 
\RMIpaper{Hilbert transforms
  and maximal functions related to variable curves}
In \RMIbook{Harmonic analysis in
  {E}uclidean spaces} ({P}roc. {S}ympos. {P}ure {M}ath., {W}illiams {C}oll.,
  {W}illiamstown, {M}ass., 1978), {P}art 1, Proc. Sympos. Pure Math., XXXV,
  Part, Amer. Math. Soc., Providence, R.I., 1979, pp.~95--98. 
%\MR{545242}

\bibitem{NagelSteinWaingerBallsAndMetricsDefinedByVectorFields}
\RMIauthor{Nagel, A. and Stein, E. and Wainger, S.} 
\RMIpaper{Balls and metrics defined by vector fields. {I}. {B}asic
  properties} 
\RMIjournal{Acta Math.} \textbf{155} (1985), no.~1-2, 103--147.
% \MR{MR793239
%  (86k:46049)}

\bibitem{NagelWaingerL2BoundednessOfHilbertTransformsMultiParameterGroup}
\RMIauthor{Nagel, A. and Wainger, S.} 
\RMIpaper{{$L^{2}$} boundedness of {H}ilbert
  transforms along surfaces and convolution operators homogeneous with respect
  to a multiple parameter group} 
\RMIjournal{Amer. J. Math.} \textbf{99} (1977), no.~4,
  761--785. 
%\MR{MR0450901 (56 \#9192)}

\bibitem{PhongSteinHilbertIntegrals}
\RMIauthor{Phong, D. and Stein, E.} 
\RMIpaper{Hilbert integrals, singular integrals, and
  {R}adon transforms. {I}} 
\RMIjournal{Acta Math.} \textbf{157} (1986), no.~1-2, 99--157.
  %\MR{857680 (88i:42028a)}

\bibitem{RicciSteinMultiparameterSingularIntegralsAndMaximalFunctions}
\RMIauthor{Ricci, F. and Stein, E.} 
\RMIpaper{Multiparameter singular integrals and maximal
  functions} 
\RMIjournal{Ann. Inst. Fourier} (Grenoble) \textbf{42} (1992), no.~3,
  637--670. %\MR{1182643 (94d:42020)}

\bibitem{RicciSteinHarmonicAnalysisOnNilpotentGroupsAndSingularIntegralsII}
\RMIauthor{Ricci, F. and Stein, E.} 
\RMIpaper{Harmonic analysis on nilpotent groups
  and singular integrals. {II}. {S}ingular kernels supported on submanifolds}
  \RMIjournal{J. Funct. Anal.} \textbf{78} (1988), no.~1, 56--84. %\MR{937632}

\bibitem{RicciSteinHarmonicAnalysisOnNilpotentGroupsAndSingularIntegralsIII}
\RMIauthor{Ricci, F. and Stein, E.} 
\RMIpaper{Harmonic analysis on nilpotent groups and singular integrals.
  {III}. {F}ractional integration along manifolds} 
\RMIjournal{J. Funct. Anal.} \textbf{86}
  (1989), no.~2, 360--389. %\MR{1021141 (90m:22027)}


\bibitem{RothschildSteinHypoellipticDifferentialOperatorsAndNilpotentGroups}
\RMIauthor{Rothschild, L. and Stein, E.} \RMIpaper{Hypoelliptic differential
  operators and nilpotent groups} \RMIjournal{Acta Math.} \textbf{137} (1976), no.~3-4,
  247--320. %\MR{MR0436223 (55 \#9171)}

\bibitem{SeegerWaingerBoundsForSingularFractionalIntegralsAndRelatedFIO}
\RMIauthor{Seeger, A. and Wainger, S.} \RMIpaper{Bounds for singular fractional
  integrals and related {F}ourier integral operators} \RMIjournal{J. Funct. Anal.}
  \textbf{199} (2003), no.~1, 48--91. %\MR{1966823 (2005d:42017)}

\bibitem{SteinMaximalFunctionsIIHomogeneousCurves}
\RMIauthor{Stein, E.} 
\RMIpaper{Maximal functions. {II}. {H}omogeneous curves}
\RMIjournal{Proc.
  Nat. Acad. Sci. U.S.A.} \textbf{73} (1976), no.~7, 2176--2177. %\MR{0420117}

\bibitem{SteinMaximalFunctionsPoissonIntegralsOnSymmetricSpaces}
\RMIauthor{Stein, E.} 
\RMIpaper{Maximal functions: {P}oisson integrals on symmetric spaces}
  \RMIjournal{Proc. Nat. Acad. Sci. U.S.A.} \textbf{73} (1976), no.~8, 2547--2549.
  %\MR{0420118}


\bibitem{SteinHarmonicAnalysis}
\RMIauthor{Stein, E.} 
\RMIbook{Harmonic analysis: real-variable methods, orthogonality, and
  oscillatory integrals}, Princeton Mathematical Series, vol.~43, Princeton
  University Press, Princeton, NJ, 1993, With the assistance of Timothy S.
  Murphy, Monographs in Harmonic Analysis, III. 
%\MR{MR1232192 (95c:42002)}

\bibitem{SteinStreetA}
\RMIauthor{Stein, E. and Street, B.} 
\RMIpaper{Multi-parameter singular {R}adon
  transforms} 
\RMIjournal{Math. Res. Lett.} \textbf{18} (2011), no.~2, 257--277.
  %\MR{2784671 (2012b:44007)}

\bibitem{SteinStreetIII}
\RMIauthor{Stein, E. and Street, B.} 
\RMIpaper{Multi-parameter singular {R}adon transforms {III}: {R}eal
  analytic surfaces} 
\RMIjournal{Adv. Math.} \textbf{229} (2012), no.~4, 2210--2238.
  %\MR{2880220}

\bibitem{SteinStreetII}
\RMIauthor{Stein, E. and Street, B.} 
\RMIpaper{Multi-parameter singular {R}adon transforms {II}: {T}he {$L^p$}
  theory} 
\RMIjournal{Adv. Math.} \textbf{248} (2013), 736--783. %\MR{3107526}

\bibitem{SteinWaingerTheEstimationOfAnIntegralArising}
\RMIauthor{Stein, E. and Wainger, S.} 
\RMIpaper{The estimation of an integral arising
  in multiplier transformations.} 
\RMIjournal{Studia Math.} \textbf{35} (1970), 101--104.
  %\MR{0265995}

\bibitem{SteinWaingerProblemsInHarmonicAnalysisRelatedToCurvature}
\RMIauthor{Stein, E. and Wainger, S.} 
\RMIpaper{Problems in harmonic analysis related to curvature}
 \RMIjournal{Bull. Amer.
  Math. Soc.} \textbf{84} (1978), no.~6, 1239--1295. 
%\MR{508453}

\bibitem{StreetMultiParameterCCBalls}
\RMIauthor{Street, B.} 
\RMIpaper{Multi-parameter {C}arnot-{C}arath\'eodory balls and the
  theorem of {F}robenius}
\RMIjournal{Rev. Mat. Iberoam.} \textbf{27} (2011), no.~2,
  645--732. 
%\MR{2848534 (2012m:53064)}

\bibitem{SteinStreetI}
\RMIauthor{Street, B.} 
\RMIpaper{Multi-parameter singular radon transforms {I}: {T}he {$L^2$}
  theory} 
\RMIjournal{J. Anal. Math.} \textbf{116} (2012), 83--162. %\MR{2892618}

\bibitem{StreetMultiParamSingInt}
\RMIauthor{Street, B.} 
\RMIbook{{M}ulti-parameter {S}ingular {I}ntegrals}, Annals of Mathematics
  Studies, vol. 189, Princeton University Press, Princeton, NJ, 2014.

\bibitem{TaoWrightLpImprovingBounds}
\RMIauthor{Tao, T. and Wright, J.} \RMIpaper{{$L^p$} improving bounds for averages along
  curves} \RMIjournal{J. Amer. Math. Soc.} \textbf{16} (2003), no.~3, 605--638. 
%\MR{1969206
 % (2004j:42005)}

\bibitem{TrevesTopologicalVectorSpaces}
\RMIauthor{Tr{\`e}ves, F.} \RMIbook{Topological vector spaces, distributions and
  kernels}, Academic Press, New York-London, 1967. 
%\MR{0225131 (37 \#726)}

%\end{thebibliography}

